Show Me What and Tell Me How: Video Synthesis via Multimodal Conditioning

Most methods for conditional video synthesis use a single modality as the condition. This comes with major limitations. For example, it is problematic for a model conditioned on an image to generate a specific motion trajectory desired by the user since there is no means to provide motion information. Conversely, language information can describe the desired motion, while not precisely defining the content of the video. This work presents a multimodal video generation framework that benefits from text and images provided jointly or separately. We leverage the recent progress in quantized representations for videos and apply a bidirectional transformer with multiple modalities as inputs to predict a discrete video representation. To improve video quality and consistency, we propose a new video token trained with self-learning and an improved mask-prediction algorithm for sampling video tokens. We introduce text augmentation to improve the robustness of the textual representation and diversity of generated videos. Our framework can incorporate various visual modalities, such as segmentation masks, drawings, and partially occluded images. It can generate much longer sequences than the one used for training. In addition, our model can extract visual information as suggested by the text prompt, e.g., "an object in image one is moving northeast", and generate corresponding videos. We run evaluations on three public datasets and a newly collected dataset labeled with facial attributes, achieving state-of-the-art generation results on all four.

==> cvpr2022/1_abstract.tex <==

\begin{abstract}
% Conditional video synthesis methods have made large strides towards the successful generation of high-fidelity videos from given textual or visual inputs. 
% However, existing efforts mainly use a single modality as the condition, limiting the potential of generative video models. 
% For example, it is difficult for a model conditioned on an image to generate a specific motion trajectory since no motion information is provided.
% On the other hand, combining visual (\emph{i.e.}, image or video) and textual modalities into one video generation framework will enable us to manipulate 
% % { \color{red} Did you mean: manipulate or learn?} 
% the generated content and motion together. 
% % \sergey{This sentence is not clear. Do you mean that if you combine, you will be able to...?}
% This work aims to tackle this challenging problem -- multimodal video generation, where synthesized videos can be conditioned on the visual modality only, the textual modality only, or both. 
% We leverage the quantized representation of images and use a bidirectional transformer to process conditional inputs to predict discrete video representation, which is then decoded to videos using a decoder. 
% To improve the quality of synthesized videos, we propose several novel techniques, using a special video token trained with self-learning, improved mask prediction, a language model for processing textual embedding, and minutes-long video synthesis. 
% Our framework can incorporate various visual modalities, including segmentation masks, drawing, and partial images.
% Besides regular conditionalthe generation, we introduce new applications, such as obtaining certain contents from the image samples by using a language description to generate videos.
% We validate our method on three public datasets and achieve the state-of-the-art generation resutls.
% % diverse and realistic generation results. 
% % { \color{red} Can you say about for example being state of the art? or how good they are?}
% We further collect and will release a multimodal facial dataset with attributes labeled to facilitate the research on multimodal video generation.
% % , which we will make it publicly available.

% Sergey: 

% Most methods for conditional video synthesis use a single modality as the condition. This comes with major limitations. For example, it is problematic for a model conditioned on an image to generate a specific motion trajectory desired by the user, since there are no means to provide motion information. Conversely, language information can provide a description of the desired motion, while not being able to precisely define the content of the video. In this work we present a multimodal video generation framework that benefits from text and images provided jointly or separately. We leverage the recent progress in quantized representation for images and apply a bidirectional transformer with multiple modalities as inputs to predict a discrete video representation. To improve video quality and consistency we propose a new video token trained with self-learning and sampled with an improved mask predict algorithm. We build robust textual representations to ensure the generated videos are consistent with the provided text. Our framework can incorporate various visual modalities, such as segmentation masks, drawings, and partially occluded images. It can generate minute-long videos. Besides, our model can extract visual information as suggested by the text prompt, e.g., ``an object in image one is moving northeast'', and generate corresponding videos. We evaluate on three public datasets and a newly collected dataset labeled with facial attributes, achieving state-of-the-art generation results on all four\footnote{We will release code, data, and trained models.}.

Most methods for conditional video synthesis use a single modality as the condition. 
This comes with major limitations. 
For example, it is problematic for a model conditioned on an image to generate a specific motion trajectory desired by the user since there is no means to provide motion information. 
Conversely, language information can describe the desired motion, while not precisely defining the content of the video. 
This work presents a multimodal video generation framework that benefits from text and images provided jointly or separately. 
We leverage the recent progress in quantized representations for videos and apply a bidirectional transformer with multiple modalities as inputs to predict a discrete video representation. 
To improve video quality and consistency, we propose a new video token trained with self-learning and an improved mask-prediction algorithm for sampling video tokens. 
We introduce text augmentation to improve the robustness of the textual representation and diversity of generated videos.
Our framework can incorporate various visual modalities, such as segmentation masks, drawings, and partially occluded images. 
It can generate much longer sequences than the one used for training.
In addition, our model can extract visual information as suggested by the text prompt, \emph{e.g.}, ``an object in image one is moving northeast'', and generate corresponding videos. We run evaluations on three public datasets and a newly collected dataset labeled with facial attributes, achieving state-of-the-art generation results on all four\footnote{Code:~\href{https://github.com/snap-research/MMVID}{\color{urlcolor}{https://github.com/snap-research/MMVID}} and~\href{https://snap-research.github.io/MMVID/}{\color{urlcolor}{Webpage}}.}.

%  We build robust textual representations to ensure the generated videos are consistent with the provided text. 
% It can generate videos several minutes long.
\end{abstract}


==> cvpr2022/2_introduction.tex <==
\section{Introduction}

% \hy{I'm a bit unsure about the term multimodal, because (1) It it not that general as the term multimodal suggests. It takes only text and images. (2) I think usualy multi suggest something >=3. I'm not sure whether current claim will be viewed as overclaims for some reviewers.}

% Generic video synthesis targets the generation of vivid and believable content using samples from a normal distribution~\cite{tulyakov2017mocogan,tian2021a}. To better control the generated content, conditional video synthesis utilizes input signals, \textit{e.g.}, images~\cite{Blattmann_2021_CVPR,Dorkenwald_2021_CVPR}, text or language~\cite{balaji2019conditional,kim2020tivgan}, and action classes~\cite{vondrick2016generating}, to synthesize videos containing the desired objects as specified by visual information, or desired actions as specified by textual information or action classes.

% Sergey

Generic video synthesis methods generate videos by sampling from a random distribution~\cite{tulyakov2017mocogan,tian2021a}. To get more control over the generated content, conditional video synthesis works utilize input signals, such as images~\cite{Blattmann_2021_CVPR,Dorkenwald_2021_CVPR}, text or language~\cite{balaji2019conditional,kim2020tivgan}, and action classes~\cite{vondrick2016generating}. This enables synthesized videos containing the desired objects as specified by visual information or desired actions as specified by textual information.
% or action classes.


Existing works on conditional video generation use only one of the possible control signals as inputs~\cite{tfgan,kim2020tivgan}. This limits the flexibility and quality of the generative process.
For example, given a screenplay we could potentially generate several movies, depending on the decisions of the director, set designer, and visual effect artist. 
In a similar way, a video generation model conditioned with a text prompt should be primed with different visual inputs.
Additionally, a generative video model conditioned on a given image should be able to learn to generate various plausible videos, which can be defined from various natural language instructions.
% A written story can result into different movies with different actors and scenes. Therefore a video generation model conditioned with a text prompt should be primed with different visual inputs. % movies, set designer and visual effect artist. In a similar way, a video generation model conditioned with a text prompt  be primed with different visual input.
% Additionally, a generative video generation model conditioned on a given image should be able to learn to generate various plausible videos, which can be defined from various natural language instructions.
% text prompts. 
For example, to generate object-centric videos with objects moving~\cite{wu2021generative}, the motion can be easily defined through a text prompt, \textit{e.g.}, ``moving in a zig-zag way,'' while the objects can be defined by visual inputs. 
Thus, an interesting yet challenging question arises: 
% \hy{I rearrange it a bit, feel free to revert it}
% \comment{
% For example, \todo{similarly to a story that can be shot into different movies with different actors and various scenery,}
% % to an audience that is being shown slides to evoke particular visual patterns as the story is being told, 
% a model conditioned with a text prompt can be primed with different visual inputs together.
% Further, to generate object-centric videos with objects moving~\cite{wu2021generative}, it is problematic to define a motion trajectory using only images as the condition.
% On the contrary, the motion can be conveniently defined through a text prompt, \textit{i.e.}, \texttt{moving in a zig-zag way}. 
% Thus, an interesting yet challenging question arises: }
\textit{Can we learn a video generation model that can support such behavior?} 
% \textit{Can we learn a video generation model that can synthesize videos using multimodal control signals?} 
% \hy{still have a negative feeling toward the multimodal term}

% To tackle the problem, we first consider what would be the most appropriate architecture for unifying multimodal samples and the process of video generation.

We tackle the question in this work and propose a new video synthesis model supporting diverse, multimodal conditioning signals. Our method consists of two phases. The \emph{first} phase obtains discrete representations from images.
% generates realistic and diverse images.
We employ an autoencoder with a quantized bottleneck, inspired by the recent success of two-stage image generation using quantized feature representations~\cite{oord2017neural,razavi2019generating,esser2020taming,zhang2021ufc}. 
The \emph{second} phase learns to generate video representations that are conditioned on the input modalities, which can then be decoded into videos using the decoder from the first stage. 
We leverage a bidirectional transformer, \emph{i.e.}, BERT~\cite{devlin2018bert}, trained with a masked sequence modeling task, that uses tokens from multimodal samples and predicts the latent representation for videos. Building such a framework requires solving several challenging problems. First, video consistency is a common problem among video generation methods. 
Second, it is necessary to ensure that the correct textual information is learned.
% and used by the transformer.
% , as it can attend to a subset of easily identifiable keywords in the prompt. 
Third, training a transformer for image synthesis is computationally demanding~\cite{chen2020generative}, an issue that is even more severe in the time domain, as a longer sequence of tokens needs to be learned. To solve these challenges, we propose the following contributions: 
% \hy{you "improve" xxx, "use" yyy to extract embedding, it will simply lead to common "lack of novelty" from lazy reviewers}
\begin{itemize}[leftmargin=1.5em]
  \setlength\itemsep{-0.25em}
  \item We introduce a bidirectional transformer with several new techniques to improve video generation: For training, we propose the video token \texttt{VID}, which is trained via self-learning and video attention, to model temporal consistency; For inference, we improve mask-predict to generate videos with improved quality.
  \item 
%   We model robust textual representation by leveraging a pretrained language model to extract textual embeddings from input language samples to generate videos that are correlated with the provided text (Fig.~\ref{fig:vox_lang}). 
  We introduce text augmentation, including text dropout and pretrained language models for extracting textual embeddings, to generate diverse videos that are correlated with the provided text.
%   to improve the robustness of textual representation and diversity of generated videos.
  \item  We explore long sequence synthesis with the transformer model to generate sequences with lengths that are much longer than the one used for training (Fig.~\ref{fig:iper}).
%   much longer sequences than the
%   for obtaining minutes-long videos, even only a few images are used for training (Fig.~\ref{fig:iper}).
\end{itemize}

We name our framework \textbf{MMVID} and show that a \textbf{M}ulti\textbf{M}odal \textbf{VID}eo generator can enable various applications. The user can show \emph{what} to generate using visual modalities and tell \emph{how} to generate with language.
We explore two settings for multimodal video generation. The first involves \textit{independent} multimodalities, such that there is no relationship between textual and visual controls (Fig.~\ref{fig:shape_vc} and Fig.~\ref{fig:vox_vc}). The second one targets \textit{dependent} multimodal generation, where we use text to obtain certain attributes from given visual controls (Fig.~\ref{fig:shape_text_dep} and Fig.~\ref{fig:vox_vc}). The latter case allows for more potential applications, in which language is not able to accurately describe certain image content that the user seeks to generate, but images can efficiently define such content. We also show our model can use diverse visual information, including segmentation masks, drawings, and partially observed images (Fig.~\ref{fig:vox_vc}).

To validate our approach extensively, we conduct experiments on \emph{four} datasets. In addition to three public datasets, we collect a new dataset, named Multimodal VoxCeleb, that includes $19,522$ videos from VoxCeleb~\cite{nagrani2020voxceleb} with $36$ manually labeled facial attributes.


% \todo{partial visual modality, different VC (draw, mask)}

% \st{Second, MMVG can use partial visual controls to inpaint or outpaint the missing visual information in the videos. Third, we can condition the motion of the generated videos on visual controls.}

% First, MMVG can synthesize videos conditioned on single or multiple modalities. Two settings can be further explored for multimodal video generation. One is \textit{independent} multimodal such that there is no relationship between textual and visual controls. Another one is \textit{dependent} multimodal generation such that we use text to obtain certain attributes from given visual controls. The dependent multimodal generation enables us for more potential applications where text is not enough to describe certain image content that we would like to generate and such content can by found from images. 
% Second, MMVG can use partial visual controls to inpaint or outpaint the missing visual information in the videos. Third, we can condition the motion of the generated videos on visual controls.


% Inspired by the recent success of two-stage image generation using quantized feature representations~\cite{oord2017neural,razavi2019generating,esser2020taming,zhang2021ufc}, we . The first is concerned with generating realistic and diverse images. The second aims at generating video representations conditioned on the input prompts. To address the first we adopt an autodencoder with a quantized bottleneck, such as VQGAN~\cite{esser2020taming}. 
% %can tokenize images, including visual controls and frames from training videos, into discrete tokens. 
% The second uses a bidirectional transformer, trained with the masked sequence modeling task, that takes visual and textual tokens and estimates the latent representation for videos, to be then rendered by the decoder. With the architecture at hand, several key problems remain challenging. The first is video consistency---a common problem in the domain of video generation. Second, training a transformer for image synthesis is computationally demanding~\cite{}, and it becomes even more so when lifted to the time domain~\cite{}. Finally, it is necessary to ensure that \emph{all} priming information is used by the transformer, as it can attend to a subset of easily identifiable keywords in the prompt. 

% First, video consistency is not considered in the architecture. We want to generate videos with consistent content and motion. Second, the training of transformer for a long sequence generation requires more GPU memory, which limits the number of frames that we can generate. Third, how to learn the transformer such that the language information is taken into consideration, rather than the categorical information from text. 

%  {the points in this paragraph should address the problems above, but it seems the points below solve other problems. Please check}
 


==> cvpr2022/3_related_work.tex <==


\section{Related Works}

\noindent\textbf{Video Generation}. For simplicity, previous works on video generation can be categorized into unconditional and conditional generation, where most of them apply similar training strategies: adversarial training with image and video discriminators~\cite{goodfellow2014generative,clark2019adversarial,TGAN2020}.
% 1. Video Generation; MoCoGAN, MoCoGAN-HD,
Research on \textit{unconditional} video generation studies how to synthesize diverse videos with input latent content or motion noise~\cite{vondrick2016generating,saito2017temporal,tulyakov2017mocogan,yushchenko2019markov,acharya2018towards,wang2020g3an,hyun2021self}. Recent efforts in this direction have achieved high resolution and high quality generation results for images and videos~\cite{kahembwe2020lower,tian2021a,clark2019adversarial}. 
% 2. Video Prediction;
On the other hand, \textit{conditional} video generation utilizes given visual or textual information for video synthesis~\cite{pan2019video,wang2020imaginator,walker2021predicting,Blattmann_2021_CVPR,Dorkenwald_2021_CVPR,ren2021flow,siarohin2021motion}. For example,
the task of video prediction uses the provided first image or a few images to generate a sequence of frames~\cite{babaeizadeh2021fitvid,denton2017unsupervised,denton2018stochastic,walker2017pose,villegas17hierchvid,villegas17mcnet,babaeizadeh2017stochastic,hsieh2018learning,byeon2018contextvp}. Similarly, text-to-video generation applies the conditional signal from text,  captions, or natural language descriptions~\cite{li2018video,marwah2017attentive,pan2017create}. TFGAN~\cite{balaji2019conditional} proposes a  multi-scale text-filter conditioning scheme for discriminators. %based on convolutional filter generation.
TiVGAN~\cite{kim2020tivgan} proposes to  generate a single image from text and synthesizes consecutive frames through further stages.
% difference
In this work, we study conditional video synthesis. However, we differ from existing methods since we address a more challenging problem: multimodal video generation. Instead of using a single modality, such as textual guidance, we show how multiple modalities can be input within a single  framework for video generation. With multimodal controls, \emph{i.e.}, textual and visual inputs, we further enhance two settings for video generation: independent and dependent multimodal inputs, in which various applications can be developed.
% based on our framework.

% First, both the textual and visual controls consist image content, attributes, or motion information that can be included in the synthesized videos. Second, the textual input can further provide guiding information of what image content or attributes from visual controls should the synthesized videos should obtain. We show examples from both settings in section xxx.





\noindent\textbf{Transformers for Video Generation}. Transformer-based networks have shown promising and often superior performance not only in natural languages processing tasks~\cite{brown2020language,radford2018improving,vaswani2017attention}, but also in computer vision related efforts~\cite{chen2020generative,dosovitskiy2020image,radford2021learning,huang2020pixel,qi2020imagebert}. Recent works prvoide promising results on conditional image generation~\cite{esser2020taming,cho2020x}, text-to-image generation~\cite{ramesh2021zero,ding2021cogview}, video generation~\cite{wu2021generative,rakhimov2020latent,Weissenborn2020Scaling,yan2021videogpt}, and text-to-video synthesis~\cite{wu2021godiva} using transformers.
Unlike existing transformer-based video generation works that focus on autoregressive training, we apply a non-autoregressive generation pipeline with a bidirectional transformer~\cite{gu2017non,gao2019masked,ghazvininejad2019mask,wang2019bert,mansimov2019generalized}. Our work is inspired by M6-UFC~\cite{zhang2021ufc}, which utilizes the non-autoregressive training for multimodal image generation and produces more diverse image generation with higher quality. Building upon M6-UFC, we further introduce training techniques for multimodal video synthesis.



==> cvpr2022/4_method.tex <==

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.98\linewidth]{cvpr2022/figure/pipeline.pdf}
%     \caption{Training and generation pipelines. (a) Data quantization. (b) Model training, inside BERT module, the green \colorbox{mygreen2}{$~^~$} triangle indicates the attention scope of \texttt{[REL]} and the blue \colorbox{myblue2}{$~^~$} triangle indicates the attention scope of \texttt{[VID]}. (c) Video extrapolation, for simplicity, each step represents a full mask-predict process instead of a single forward pass of the transformer. (d) Video interpolation.}
%     % \hy{I think the figure is not clear and self-explanatory enough without any prior to the task.}
%     \label{fig:pipeline}
% \end{figure*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{cvpr2022/figure/pipeline.pdf}
    \caption{\textbf{Pipeline} for training and inference. (a) Data quantization. (b) Model training. Within the BERT module, the {green} and {blue} triangles indicate the attention scopes of \colorbox{mygreen2}{\texttt{[REL]}} and \colorbox{myblue2}{\texttt{[VID]}}, respectively. (c) Video extrapolation. For simplicity, each step represents a full mask-predict process instead of a single forward pass of the transformer. (d) Video interpolation.    }
    \label{fig:pipeline}
\end{figure*}

\section{Methods}
Our framework for multimodal video generation is a two-stage image generation method. It uses discrete feature representations~\cite{oord2017neural,razavi2019generating,esser2020taming,zhang2021ufc}. During the \emph{first} stage we train an autoencoder (with encoder $E$ and decoder $D$) that has the same architecture as the one from VQGAN~\cite{esser2020taming} to obtain a quantized representation for images. 
% Let the codebook represented by $\mathcal{Z}$.
% The autoencoder can obtain a codebook $\mathcal{Z}$ with context-rich visual parts for each image. 
Given a real video clip defined as $\mathbf{v}=\{\mathbf{x}_1, \mathbf{x}_2, \cdots, \mathbf{x}_T\}$ with $\mathbf{x}_t\in\mathbb{R}^{H\times W\times 3}$, we get a quantized representation of the video defined as $\mathbf{z}=\{\mathbf{z}_1, \mathbf{z}_2, \cdots, \mathbf{z}_T\}$, where $\mathbf{z}_t = {q}(E(\mathbf{x}_t))\in\mathbb{N}_1^{h\times w}$. ${q}(\cdot)$ denotes the quantization operation and $\mathbb{N}_1$ indicates a set of positive integers.
% \vspace{-0.1in}

During the \emph{second} stage we learn a bidirectional transformer for modeling the correlation between multimodal controls and the learned vector quantization representation of a video. 
Specifically, we concatenate the tokens from the multimodal inputs and the target video as a sequence to train the transformer.
% Inspired by DALL-E~\cite{ramesh2021zero}, we model the full concatenated sequence of controls and target videos by a transformer. 
Tensors obtained from an image and video must be vectorized for concatenation. We do so using the reshape operation ($\texttt{Reshape}$).
% Therefore, we have an image tensor $\mathbf{z}_t$ reshaped into a single-index tensor as $[z_t^{(1)},\cdots,z_t^{(hw)}]$. Similarly, a tensor $\mathbf{z}$ from video can be reshaped as $\texttt{Reshape}(\mathbf{z})=[z^{(1)},\cdots,z^{(hwT)}]$.
Therefore, we have a video tensor $\mathbf{z}$ reshaped into a single-index tensor as $\texttt{Reshape}(\mathbf{z})=[z^{(1)},\cdots,z^{(hwT)}]$.
For simplicity of notation, we define $\mathbf{z}\equiv\texttt{Reshape}(\mathbf{z})$.
To train the non-autogressive transformer (BERT) on video tokens, we employ three tasks: Masked Sequence Modeling (MSM),  RELevance estimation (REL), and VIDeo consistency estimation (VID). During inference, samples are generated via an iterative algorithm based on mask-predict~\cite{ghazvininejad2019mask}, which is simulated by the MSM task during training. The REL and VID tasks regularize the model to synthesize videos that are relevant to the multimodal signals and are temporally consistent.
In the following two sections we present each task.
% Thus tensor $\mathbf{z}$ needs to be vectorized. Different serialization methods can be used and we use reshape for simplicity,
% % $\mathbf{z}$ can be reshaped into a single-index tensor $[z_1^{(1)},\cdots,z_1^{(hw)},\cdots,z_T^{(hw)}]$.
% $\mathbf{z}_t$ can be reshaped into a single-index tensor $[z_t^{(1)},\cdots,z_t^{(hw)}]$, and similarly, $\texttt{Reshape}(\mathbf{z})=[z^{(1)},\cdots,z^{(hwT)}]$. With a slight abuse of notation, we also denote the serialized discrete representation as $\mathbf{z}$.

% Formally, given a real video clip as $\mathbf{v} = \{\mathbf{x}_1, \mathbf{x}_2, \cdots, \mathbf{x}_n\}$ with $\mathbf{x}_i\in\mathbb{R}^{H\times W\times 3}$ and a VQGAN with encoder $E$ and decoder $D$, we can get the quantized representation of a video as $\mathbf{z} = \{\mathbf{z}_1, \mathbf{z}_2, \cdots, \mathbf{z}_n\}$. $\mathbf{z}_i$ is obtained by $\mathbf{z}_i = E(\mathbf{x}_i)$

% The generated video sequence $\tilde{\mathbf{v}}$ is given by $\tilde{\mathbf{v}} = \{\tilde{\mathbf{x}}_1, \tilde{\mathbf{x}}_2, \cdots, \tilde{\mathbf{x}}_n\}$

% Formally, given a real video clip as $\mathbf{v} = \{\mathbf{x}_1, \mathbf{x}_2, \cdots, \mathbf{x}_T\}$ with $\mathbf{x}_t\in\mathbb{R}^{H\times W\times 3}$ and a VQGAN with encoder $E$ and decoder $D$, we can get the quantized representation of a video as $\mathbf{z} = \{\mathbf{z}_1, \mathbf{z}_2, \cdots, \mathbf{z}_T\}$. $\mathbf{z}_t$ is obtained by $\mathbf{z}_t = \mathbf{q}(E(\mathbf{x}_t)) \in \mathbb{N}_0^{h\times w}$, where $\mathbf{q}(\cdot)$ is the quantization operation and $\mathbb{N}_0$ is the set of non-negative integers \sergey{why q is mathbf?}. The generated video sequence $\tilde{\mathbf{v}}$ is given by $\tilde{\mathbf{v}} = \{\tilde{\mathbf{x}}_1, \tilde{\mathbf{x}}_2, \cdots, \tilde{\mathbf{x}}_T\}$.



% The generated video sequence $\tilde{\mathbf{v}}$ is given by $\tilde{\mathbf{v}} = \{\tilde{\mathbf{x}}_1, \tilde{\mathbf{x}}_2, \cdots, \tilde{\mathbf{x}}_T\}$.

% The main idea of our video generation model is to train a BERT model on video tokens with masked sequence modeling (MSM) two additional estimation tasks: relevance estimation (REL), and video consistency estimation (VID). During inference time, samples are generated via an iterative algorithm similar to mask-predict~\cite{ghazvininejad2019mask}, which is simulated by the masked sequence modeling task during training. The estimation tasks regularize the model to synthesize videos that are relevant to the control signals and are also temporally consistent.
% We explain each task as follows.

\subsection{Masked Sequence Modeling with Relevance}\label{sec:msm} 
\noindent\textbf{Masked Sequence Modeling}. The MSM task is similar to a conditional masked language model~\cite{ghazvininejad2019mask}. It is essential for the non-autoregressive model to learn bidirectional representations and enables parallel generation (mask-predict). Inspired by M6-UFC~\cite{zhang2021ufc} and VIMPAC~\cite{tan2021vimpac}, we consider five masking strategies: (I) i.i.d. masking, \emph{i.e.}, randomly masking video tokens according to a Bernoulli distribution; %with probability $0.8$;
% , where the probability $p_\text{MSM}^\text{Ber}$ is given as $p_\text{MSM}^\text{Ber}=0.8$; 
(II) masking all tokens; (III) block masking~\cite{tan2021vimpac}, which masks continuous tokens inside spatio-temporal blocks; (IV) the negation of block masking, which preserves the spatio-temporal block and masks the rest of the tokens; (V) randomly keeping some frames (optional). Strategies I and II are designed to simulate mask-predict sampling (the strategy chosen most of the time). 
% During training, strategy I is chosen most of the time since it simulates the input sequences used in mask-predict. 
Strategy II helps the model learn to generate from a fully masked sequence in the first step of mask-predict. Strategies III - V can be used as Preservation  Control  (PC)  for preservation tasks, which enable the use of partial images as input (Figs.~\ref{fig:shape_vc},~\ref{fig:vox_vc}) and performing long sequence generation (Fig.~\ref{fig:iper}).
% , video inpainting and outpainting. 
% Denoting the masking indices as set $\mathcal{M}$, the masked sequence as ${\mathbf{z}^m}$ and control sequence as $\mathbf{c}$, the masked sequence modeling task minimizes the softmax cross-entropy loss
The MSM task minimizes the softmax cross-entropy loss $\mathcal{L}_\text{MSM}$ as follows:
% $\mathcal{L}_\text{MSM}=\frac{1}{|\mathcal{M}|}\sum_{i\in\mathcal{M}}{-\log{P(z^{(i)}|{\mathbf{z}^m}, \mathbf{c})}}$.
\begin{equation}
% \begin{split}
\small
\mathcal{L}_\text{MSM}=-\frac{1}{|\mathcal{M}|}\sum_{i\in\mathcal{M}}{\log{P(z^{(i)}|{\mathbf{z}^m}, \mathbf{c})}},
%  \mathcal{L}_{D_p}=&\mathbb{E}_{\mathbf{x},\mathbf{f}}[\log D_p(\mathbf{x}_t,\mathbf{f}_t)]+\\
%  &\mathbb{E}_{\mathbf{x}}[\log(1-D_p(\mathbf{x}_t,G(\tilde{\mathbf{x}}_t))],
% \end{split}
\label{eq:msm}
\end{equation}
where $\mathcal{M}$ is the masking indices, ${\mathbf{z}^m}$ is the masked sequence, and $\mathbf{c}$ denotes the control sequence.


\noindent\textbf{Relevance Estimation}. To encourage the transformer to learn the correlation between multimodal inputs and target videos, we prepend a special token \texttt{REL} that is similar to the one used in M6-UFC~\cite{zhang2021ufc}  to the whole sequence, and learn a binary classifier to classify positive and negative sequences. The positive sequence is the same as the sequence used in the MSM task so that we can reuse the same transformer in the forward pass. The negative sequence is constructed by swapping the condition signals along the batch dimension. This swapping does not guarantee constructing strictly negative samples. Nevertheless, we still find it is good enough to make the model learn relevance in practice.
% We also experiment with sampling negative samples from the dataset instead of swapping within the batch. We empirically find that the simple swapping strategy gives slightly better performance when model converged.
% Denoting the swapped control sequence as $\bar{\mathbf{c}}$, the relevance estimation task minimizes the binary cross-entropy loss
The loss function $\mathcal{L}_\text{REL}$ for the relevance task is given by:
% $\mathcal{L}_\text{REL}=-\log{P(1|{\mathbf{z}^m}, \mathbf{c})}-\log{P(0|{\mathbf{z}^m}, \bar{\mathbf{c}})}$.
\begin{equation}
\small
\mathcal{L}_\text{REL}=-\log{P(1|{\mathbf{z}^m}, \mathbf{c})}-\log{P(0|{\mathbf{z}^m}, \bar{\mathbf{c}})},
\label{eq:rel}
\end{equation}
where $\bar{\mathbf{c}}$ denotes the swapped control sequence.

% We also tried to sample new negative samples from the dataset instead of swapping within the batch. Such strategy causes the model to converge slower since it introduces more training samples within the same number of iterations but when the model converges it gives slightly better performance.


\subsection{Video Consistency Estimation}
To further regularize the model to generate temporally consistent videos, we introduce the video consistency estimation task. Similar to \texttt{REL}, we use a special token \texttt{VID} to classify positive and negative sequences.

\noindent\textbf{Video Attention}. The VID task focuses on video token sequences. Thus, we place the \texttt{VID} token between the control and target sequences. We apply a mask to BERT to blind the scope of the \texttt{VID} token from the control signals so it only calculates attention from the tokens of the target videos. The positive sequence is the same one used in MSM and REL tasks. The negative sequence is obtained by performing negative augmentation on videos to construct samples that do not have temporally consistent motion or content.
% and the negative sequence is assembled by the (positive) control sequence and masked negatively augmented target sequence.
% It can be seen that, without video scope masking, the transformer will be confused by the prepended positive control signals.

\noindent\textbf{Negative Video Augmentation}. We employ four strategies to augment negative video sequences: (I) \emph{frame swapping} -- a random frame is replaced by using a frame from another video;
% for each sequence swap one frame with another video; 
(II) \emph{frame shuffling} -- frames within a sequence are shuffled; 
(III) \emph{color jittering} -- randomly changing the color of one frame; (IV) \emph{affine transform} -- randomly applying an affine transformation on one frame. All augmentations are performed in image space.
With $\bar{\mathbf{z}}$ denoting the video sequence after augmentation, the loss $\mathcal{L}_\text{VID}$ for the VID task is:
% Denoting the video sequence after augmentation as $\bar{\mathbf{z}}$, the video consistency estimation task minimizes the binary cross-entropy loss
% $\mathcal{L}_\text{VID}=-\log{P(1|{\mathbf{z}^m}, \mathbf{c})}-\log{P(0|{\bar{\mathbf{z}}^m}, {\mathbf{c}})}$.
\begin{equation}
\small
\mathcal{L}_\text{VID}=-\log{P(1|{\mathbf{z}^m}, \mathbf{c})}-\log{P(0|{\bar{\mathbf{z}}^m}, {\mathbf{c}})}.
\label{eq:vid}
\end{equation}
% \noindent We construct the negative sequence for VID as $\texttt{Cat}(\textbf{c},\bar{\textbf{z}}^m)$ with positive control $\textbf{c}$ to encourage the model to further ``purify'' the features of relevant sequences to be video consistent. %Thus, it is important to blind the \texttt{VID} token's scope
Overall, the full objective is $\mathcal{L}=\lambda_\text{MSM}\mathcal{L}_\text{MSM} + \lambda_\text{REL}\mathcal{L}_\text{REL} + \lambda_\text{VID}\mathcal{L}_\text{VID}$, where $\lambda$s balances the losses.


% {\color{red} Ok what I said since it Lacked a connection ?}
% , while 
% We introduce an additional fully-connected layer to match the feature dimension with our transformer model.
% We do this by replacing the lookup table text embeddings with the weighted sum of last-layer feature vectors of the language model $Lang$, $\textbf{e}_\text{TC}=\texttt{MLP}(Lang(\text{text}))$, the $\texttt{MLP}$ is introduced to align the language model's feature dimension with that of our transformer model. $\textbf{e}_{TC}$ then occupies only one token's length.
% Note that the original text tokenizer already has some capability to handle out-of-distribution text prompt, but it might not be able to handle synonymous without common root. For example, CLIP's~\cite{radford2021learning} Simple tokenizer encodes `eyeglasses' as $[5034, 6116]$, `glasses' as $[6116]$, but `spectacles' as $[7242, 840]$.
% To let the model be more robust to textual information, we consider using a fixed \emph{pretrained} language model (RoBERTa~\cite{liu2019roberta}) rather than learning textual embeddings of text tokens from scratch. We do this by replacing the lookup table text embeddings with the weighted sum of last-layer feature vectors of the language model $Lang$, $\textbf{e}_\text{TC}=\texttt{MLP}(Lang(\text{text}))$, the $\texttt{MLP}$ is introduced to align the language model's feature dimension with that of our transformer model. $\textbf{e}_{TC}$ then occupies only one token's length.
% Note that the original text tokenizer already has some capability to handle out-of-distribution text prompt, but it might not be able to handle synonymous without common root. For example, CLIP's~\cite{radford2021learning} Simple tokenizer encodes `eyeglasses' as $[5034, 6116]$, `glasses' as $[6116]$, but `spectacles' as $[7242, 840]$.


\subsection{Improved Mask-Predict for Video Generation}
We employ mask-predict~\cite{ghazvininejad2019mask} during inference, which iteratively remasks and repredicts low-confidence tokens by starting from a fully-masked sequence. We chose it because it 
can be used with our bidirectional transformer, as the length of the target sequence is fixed. In addition, mask predict provides several benefits. First, it allows efficient parallel sampling of tokens in a sequence. Second, the unrolling iterations from mask-predict enable direct optimization on synthesized samples, which can reduce exposure bias~\cite{ranzato2015sequence}. Third, information comes from both directions, which makes the generated videos more consistent.
% since it enables parallel sampling of tokens in a sequence. Besides efficient inference, unrolling mask-prediction iterations enables direct optimization on synthesized samples, which potentially reduces exposure bias~\cite{ranzato2015sequence}.  During inference time, the information comes from both directions, which makes the video more consistent. Moreover, the length of target sequence is fixed, which makes it naturally fit for mask-prediction.
% We build upon the original mask-predict algorithm, but adopt changes including noise annealing multinomial sampling, and early stopping, and a new scheme of annealing masks.

% Starting from a fully-masked sequence, mask-predict algorithm~\cite{ghazvininejad2019mask} realizes parallel sampling by iteratively remask and repredict unconfident tokens. 
We build our sampling algorithm based on the original mask-predict~\cite{ghazvininejad2019mask} with two improvements:
% We build our sampling algorithm upon original mask-predict by adopting improvements including: 
(I) noise-annealing multinomial sampling, \ie, adding noise during remasking; (II) a new scheme for mask annealing, \ie, using a piecewise linear annealing scheme to prevent the generated motion from being washed out after too many steps of mask-predict. We also apply a beam search from M6-UFC~\cite{zhang2021ufc}. In Alg.~\ref{alg:mask_predict}, the transformer ($\texttt{BERT}$) takes input tokens $\mathbf{z}_{in}$ and outputs score $s$ and the logits $\tilde{\mathbf{p}}$ for all target tokens. At each mask-predict iteration, we sample tokens with $\texttt{SampleToken}$ that returns a predicted token $\mathbf{z}_{out}$ and 
% which also returns 
a vector $\mathbf{y}$ containing its probabilities (unnormalized).
% of each predicted token (unnormalized). 
$\texttt{SampleToken}$ also accepts a scalar $\sigma$ that indicates the noise level to be added during the token sampling process. $\texttt{SampleMask}(\mathbf{y},\mathbf{m},N-n)$ remasks $n$ tokens from a total of $N$ tokens according to the multinomial defined by the normalized $\mathbf{y}$, while ensuring tokens with $\mathbf{m}=1$ are always preserved. $\mathbf{z}_\phi$ denotes the fully-masked sequence. The functions $\texttt{SampleToken}$, $\texttt{SampleMask}$ and the schedules of $n^{(i)}$ and $\sigma^{(i)}$ are shown in Appendix.
% $m$ is mask of same shape as $\mathbf{z}$ where $1$ indicates keeping the token. $\odot$ is elementwise product. Masking sampling function $\texttt{sample}(p,m,n)$ samples $n$ tokens from the multinomial distribution defined by $p$ and assigns value $1$ to the corresponding entries in $m$. The sampling process assures that tokens with $m=1$ will not be sampled. $n^{(i)}$ is the number of tokens to mask at iteration-$i$. 
% $\sigma$\todo{ not introduced}
% \begin{algorithm}[h]
% \caption{Improved Mask-Predict for Video Generation}
% \label{alg:mask_predict}
% \begin{algorithmic}[1]
%     \State $m_\text{PC} \leftarrow m^{(0)}_\text{PC}$ init
%     \State $\mathbf{z}_{in} \leftarrow \mathbf{z}^{(0)}_{in}$ init
%     \State $\mathbf{z}_{out}, p, s \leftarrow \texttt{BERT}(z_{in}, \sigma^{(1)})$
%     \State $\mathbf{z}_{out} \leftarrow m_\text{PC}\odot \mathbf{z}_{in} + (1-m_\text{PC}) \odot \mathbf{z}_{out}$
%     \For{$i \in \{2, ..., M\}$}
%         \For{$b \in \{1, ..., B\}$}
%             \State $m^b \leftarrow \texttt{sample}(p, m_\text{PC}, N-n^{(i)})$
%             \State $\mathbf{z}^b_{in} \leftarrow m^b\odot \mathbf{z}_{out} + (1-m^b) \odot \mathbf{z}_{\phi}$
%             \State $\mathbf{z}^b_{out}, p^b, s^b \leftarrow \texttt{BERT}(\mathbf{z}^b_{in}, \sigma^{(i)})$
%         \EndFor
%         \State $b^* \leftarrow \argmax_b(s^b)$
%         \State $p \leftarrow p^{b^*}$
%         \State $z_{out} \leftarrow z_{out}^{b^*}$
%     \EndFor
%     \State \Return $z_{out}$
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[h]
% \caption{SampleToken}
% \label{alg:sample}
% \begin{algorithmic}[1]
%     \Require logit $\tilde{\mathbf{P}}$, noise level $\sigma$
%     \State $\mathbf{g} \leftarrow \text{Gumbel}(0, 1) ~~i.i.d.$
%     \State $\mathbf{p} \leftarrow \text{Softmax}(\tilde{\mathbf{p}}+\sigma\mathbf{g})$
%     \State $\mathbf{z} \leftarrow \text{Multinomial}(\mathbf{p})$
%     \State $\mathbf{y} \leftarrow \text{Gather}(\mathbf{p}, \mathbf{z})$
%     % \State $\mathbf{y} \leftarrow \text{Diag}(\mathbf{p} \text{onehot}(\mathbf{z}))$
%     \State \Return $\mathbf{z}$, $\mathbf{y}$
% \end{algorithmic}
% \end{algorithm}
\begin{algorithm}[h]
\caption{Improved Mask-Predict for Video Generation}
\label{alg:mask_predict}
\begin{algorithmic}[1]
    \Require Initial PC mask $\mathbf{m}_\text{PC}$ and initial token $\mathbf{z}_{in}$.
    % \State $\mathbf{m}_\text{PC} \leftarrow \mathbf{m}^{(0)}_\text{PC}$ initialize
    % \State $\mathbf{z}_{in} \leftarrow \mathbf{z}^{(0)}_{in}$ initialize
    \State $\tilde{\mathbf{p}}, s \leftarrow \texttt{BERT}(\mathbf{z}_{in})$
    \State $\mathbf{z}_{out}, \mathbf{y} \leftarrow \texttt{SampleToken}(\tilde{\mathbf{p}}, \sigma^{(1)})$
    \State $\mathbf{z}_{out} \leftarrow \mathbf{m}_\text{PC}\odot \mathbf{z}_{in} + (1-\mathbf{m}_\text{PC}) \odot  \mathbf{z}_{out}$ \Comment{\textcolor{commentcolor}{PC}}
    \For{$i \in \{2, ..., L\}$} \Comment{\textcolor{commentcolor}{main loop}}
        \For{$b \in \{1, ..., B\}$} \Comment{\textcolor{commentcolor}{beam search}}
            \State $\mathbf{m}^b \leftarrow \texttt{SampleMask}(\mathbf{y}, \mathbf{m}_\text{PC}, N-n^{(i)})$ %\Comment{\textcolor{commentcolor}{PC}}
            \State $\mathbf{z}^b_{in} \leftarrow \mathbf{m}^b\odot \mathbf{z}_{out} + (1-\mathbf{m}^b) \odot \mathbf{z}_{\phi}$ \Comment{\textcolor{commentcolor}{remask}}
            \State $\tilde{\mathbf{p}}^b, s^b \leftarrow \texttt{BERT}(\mathbf{z}^b_{in})$ \Comment{\textcolor{commentcolor}{repredict}}
        \EndFor
        \State $b^* \leftarrow \argmax_b(s^b)$
        % \State $\tilde{\mathbf{p}} \leftarrow \tilde{\mathbf{p}}^{b^*}$
        \State $\mathbf{z}_{out}, \mathbf{y} \leftarrow \texttt{SampleToken}(\tilde{\mathbf{p}}^{b^*}, \sigma^{(i)})$
        % \State $\mathbf{y} \leftarrow \mathbf{y}^{b^*}$
        % \State $\mathbf{z}_{out} \leftarrow \mathbf{z}_{out}^{b^*}$
    \EndFor
    \State \Return $\mathbf{z}_{out}$
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[h]
% \caption{Improved Mask-Predict for Video Generation}
% \label{alg:mask_predict}
% \begin{algorithmic}[1]
%     \State $\mathbf{m}_\text{PC} \leftarrow \mathbf{m}^{(0)}_\text{PC}$ initialize
%     \State $\mathbf{z}_{in} \leftarrow \mathbf{z}^{(0)}_{in}$ initialize
%     \State $\mathbf{z}_{out}, \tilde{\mathbf{p}}, s \leftarrow \texttt{BERT}(\mathbf{z}_{in})$
%     \State $\mathbf{z}_{out} \leftarrow \mathbf{m}_\text{PC}\odot \mathbf{z}_{in} + (1-\mathbf{m}_\text{PC}) \odot \mathbf{z}_{out}$
%     \For{$i \in \{2, ..., L\}$}
%         \For{$b \in \{1, ..., B\}$}
%             \State $\mathbf{g} \leftarrow \text{Gumbel}(0, 1) i.i.d.$
%             \State $\mathbf{p} \leftarrow \text{Softmax}(\tilde{\mathbf{p}}+\sigma^{(i)}\mathbf{g})$
%             \State $\mathbf{m}^b \leftarrow \text{Sample}(\mathbf{p}, \mathbf{m}_\text{PC}, N-n^{(i)})$
%             \State $\mathbf{z}^b_{in} \leftarrow \mathbf{m}^b\odot \mathbf{z}_{out} + (1-\mathbf{m}^b) \odot \mathbf{z}_{\phi}$
%             \State $\mathbf{z}^b_{out}, \tilde{\mathbf{p}}^b, s^b \leftarrow \texttt{BERT}(\mathbf{z}^b_{in})$
%         \EndFor
%         \State $b^* \leftarrow \argmax_b(s^b)$
%         \State $\tilde{\mathbf{p}} \leftarrow \tilde{\mathbf{p}}^{b^*}$
%         \State $\mathbf{z}_{out} \leftarrow \mathbf{z}_{out}^{b^*}$
%     \EndFor
%     \State \Return $\mathbf{z}_{out}$
% \end{algorithmic}
% \end{algorithm}


% How is score computed? determine mixing ratio under different cases like counterfactual
% How is ni determined? how to add noise in sample?
% noise: add log(log(u)) to logits, then gather prob v.s. add noise to gathered prob?
\subsection{Text Augmentation}
We study two augmentation methods. First, we randomly drop sentences from the input text to avoid memorizing certain word combinations.
Second, we apply a fixed \emph{pretrained} language model, \emph{i.e.}, RoBERTa~\cite{liu2019roberta}, rather than learning text token embeddings in a lookup table from scratch, to let the model be more robust for input textual information.
% To let the model be more robust for input textual information, we use a fixed \emph{pretrained} language model, \emph{i.e.}, RoBERTa~\cite{liu2019roberta}, rather than learning textual embedding of text tokens from scratch.
% We replace the text embedding obtained from a lookup table with the features calculated from the language model.
The features of text tokens are obtained from an additional multilayer perceptron (MLP) appended after the language model that matches the vector dimension with BERT. 
The features are converted to a weighted sum to get the final embedding of the input text.
With the language model, the video generation framework is more robust for out-of-distribution text prompts. When using the tokenizer from an existing work~\cite{radford2021learning}, we observed that it might not properly handle synonyms without a common root (Fig.~\ref{fig:vox_lang}). %We address this issue in the next section.
\subsection{Long Sequence Generation}
Due to the inherent preservation control mechanism during training (strategy V in the MSM task), we can generate sequences with many more frames than the model is trained with via interpolation or extrapolation. \textbf{Interpolation} is conducted by generating the intermediate frames between given frames. As illustrated by Fig.~\ref{fig:pipeline} (d), we place $\mathbf{z}_1$ and $\mathbf{z}_2$ at the positions of frames 1 and 3 to serve as preservation controls, \ie, they are kept the same during mask-predict iterations, and we can interpolate a frame between them.
\textbf{Extrapolation} is similar to interpolation, except we condition the model on previous frames to generate the next frames. As illustrated in Fig.~\ref{fig:pipeline} (c), this process can be iterated a number of times to generate longer videos.


==> cvpr2022/5_experiments.tex <==
\section{Experiments}
% In this section, we discuss the experimental and comparison results on four datasets. More results for generated videos are shown in the \emph{Supplementary Materials}.
% \subsection{Basic Setting}
\noindent \textbf{Datasets.} We show experiments on the following datasets.
\begin{itemize}[leftmargin=1em]
  \setlength\itemsep{-0.25em}
    \item \textbf{Shapes} is proposed by TFGAN~\cite{tfgan} for text-to-video generation. Each video shows one object (a geometric shape with specified color and size) displayed in a textured moving background. The motion of an object is described by a text and the background is moving in a random way. There are $30$K videos with size $64\times64$.
    \item \textbf{MUG}~\cite{aifanti2010mug} contains $52$ actors performing $6$ different facial expressions. %$1462$ videos with
    % which are anger, disgust, fear, happiness, sadness, and surprise. 
    We also provide gender labels for the actors. For a fair comparison, we obtain text descriptions by following TiVGAN~\cite{kim2020tivgan}. We run experiments on $1039$ videos with resolution $128\times128$.
    \item \textbf{iPER}~\cite{liu2019liquid} consists of $206$ videos of $30$ subjects wearing different clothes performing an A-pose and random actions. Experiments are conducted with size $128\times128$.
    \item \textbf{Multimodal VoxCeleb} is a new dataset for multimodal video generation. We first obtain $19,522$ videos from  VoxCeleb~\cite{nagrani2020voxceleb} after performing  pre-processing~\cite{Siarohin_2019_NeurIPS}. Second, we manually label $36$ facial attributes described in CelebA~\cite{liu2015faceattributes} for each video. Third, we use a probabilistic context-free grammar to generate language descriptions~\cite{xia2021tedigan}. Finally, we run APDrawingGAN~\cite{YiLLR20} to get artistic portrait drawings and utilize face-parsing~\cite{yu2021bisenet} to produce segmentation masks. 
    % The dataset will be released.
    % VoxCeleb dataset~\cite{nagrani2020voxceleb} contains 22496 videos extracted from YouTube. We use the same pre-processing pipeline as in~\cite{Siarohin_2019_NeurIPS} and obtain 19522 sequences for training. The original VoxCeleb dataset has no textual descriptions or attribute annotations, so we manually labeled 40 facial attributes similar to CelebA~\cite{liu2015faceattributes}. Similar to the Multi-Modal-CelebA-HQ dataset~\cite{xia2021tedigan}, we use a probabilistic context-free grammar model to generate textual descriptions. We run APDrawingGAN~\cite{YiLLR20} to generate artistic portrait drawings and we use face-parsing\footnote{\url{https://github.com/VisionSystemsInc/face-parsing.PyTorch}}\todo{citation} to produce segmentation masks.
\end{itemize}
% \noindent \textbf{Shapes} is proposed by TFGAN~\cite{tfgan} for text-to-video generation. Each video shows one object (a geometric shape with specified color and size) displayed in a textured moving background. Motion of an object is described by a text and background is moving in a random way. There are $30$K videos with frame size as $64\times64$.

% \noindent \textbf{MUG}~\cite{aifanti2010mug} contains $52$ actors performing $6$ different facial expressions. We also provide gender labels for the actors. For a fair comparison, we obtain text descriptions by following TiVGAN~\cite{kim2020tivgan}. We run experiments on $1039$ videos with resolution of $128\times128$.

% \noindent \textbf{iPER}~\cite{liu2019liquid} consists of $206$ videos of $30$ subjects wear different clothes performing an A-pose and random actions. Experiments are conducted at size of $128\times128$.

% \noindent \textbf{Multimodal VoxCeleb} is a new dataset for multimodal video generation. We first obtain $19522$ videos from  VoxCeleb~\cite{nagrani2020voxceleb} after performing  pre-processing~\cite{Siarohin_2019_NeurIPS}. Second, we manually label $36$ facial attributes that described in CelebA~\cite{liu2015faceattributes} for each video. Third, we use a probabilistic context-free grammar model to generate language description~\cite{xia2021tedigan}. Finally, we run APDrawingGAN~\cite{YiLLR20} to get artistic portrait drawings and utilize face-parsing~\cite{yu2021bisenet} to produce segmentation masks. The dataset will be released.

% We then present various applications for multimodal video generation on these datasets.
\noindent \textbf{Baseline Methods}. We run TFGAN~\cite{tfgan} on Shapes, MUG, and Multimodal VoxCeleb datases for comparison of text-to-video synthesis. We also compare our approach with TiVGAN~\cite{kim2020tivgan} on MUG. 
Additionally, we unify the autoregressive transformer of DALL-E~\cite{ramesh2021zero} and the autoencoder from VQGAN (the same one used in our method) in a multimodal video generative model. We name the strong baseline as {\bf A}uto{\bf R}egressive {\bf T}ransformer for {\bf V}ideo generation (\textbf{ART-V}) and compare it with our bidirectional transformer for predicting video tokens. 
% text-to-video generation as well as taking visual controls. 
% We use the same first-stage VQGAN models as our model, and 
% We train ART-V with next-token-prediction objective on concatenated $\texttt{Cat}(\textbf{c},\textbf{z})$ \texttt{(textual, visual, target-visual)} token sequences.
% We train ART-V with next-token-prediction objective on concatenated $\texttt{Cat}(\textbf{c},\textbf{z})$ token sequences of input controls and target videos.
We train ART-V with the next-token-prediction objective on concatenated token sequences obtained from input controls and target videos.
% The resulting model serves as a strong baseline, which we call {\bf A}uto{\bf R}egressive {\bf T}ransformer for {\bf V}ideo generation (ART-V). For each dataset, we finetune a VQGAN model (pretrained on ImageNet, with $f=16$ and $|\mathcal{Z}|=1024$) at each resolution.

\noindent \textbf{Evaluation Metrics}. 
We follow the metrics from existing works on Shapes and MUG to get a fair comparison. Specifically, we compute classification accuracy on Shapes and MUG and Inception Score (IS)~\cite{salimans2016improved} on MUG. 
% We also report cla
% For Shapes, we compute classification accuracy to get a fair comparison with existing works. For MUG dataset, we report Inception Scores (IS)~\cite{salimans2016improved} and additional classification accuracies. 
On Multimodal VoxCeleb and iPER datasets, we report Fr\'{e}chet Video Distances (FVD)~\cite{unterthiner2018towards} that is computed from $2048$ samples, and Precision-Recall Distribution (PRD) ($F_{8}$ and $F_{1/8}$) for diversity~\cite{precision_recall_distributions}. We further report the CLIP score~\cite{radford2021learning} for calculating the cosine similarity between textual inputs and the generated videos on Multimodal VoxCeleb. % LPIPS score~\cite{zhang2018unreasonable,choi2020starganv2}
% \todo{we might need to introduce the metrics about what they do}
% We evaluate the text-video relevance by CLIP score, which is computed as the cosine similarity of text embedding and image embedding of the first frame given by the pretrained CLIP model~\cite{radford2021learning}. We also compute the FVD score~\cite{unterthiner2018towards} from 2048 samples. Sample diversity is evaluated by the precision and recall distribution ($F_{8}$ and $F_{1/8}$)~\cite{precision_recall_distributions}. The  Human evaluation is the portion of AMTuker's preference given a pairwise comparison of samples.
% \begin{figure}[t]
% \centering
% \begin{subfigure}[t] {1\linewidth}
%     \centering
%     \setlength{\tabcolsep}{0\linewidth}
%     \begin{tabular}{L{1\linewidth}}
%     \rowcolor{hlrowcolor}
%     \linespread{0.5}\noindent
%     \small{\scriptsize A large blue circle is moving in a straight line towards south.}
%     \end{tabular}
%     \includegraphics[width=1\linewidth]{cvpr2022/figure/shape_txt_all_color_new2.pdf}
%     \caption{Sample results on the \textbf{Shapes} dataset. TFGAN fails to generate sequences with clear shapes and complicated backgrounds.}
%     \label{fig:shape_txt_all}
% \end{subfigure}\hfill
% \begin{subfigure}[t] {1\linewidth}
%     \centering
%     \setlength{\tabcolsep}{0\linewidth}
%     \begin{tabular}{L{1\linewidth}}
%     \rowcolor{hlrowcolor}
%     \linespread{0.5}\noindent
%     \small{\scriptsize A woman is making a surprise face.}
%     \end{tabular}
%     \includegraphics[width=\linewidth]{cvpr2022/figure/mug_txt_all_5_color_new2.pdf}
%     \caption{Sample results on \textbf{MUG} dataset.
%     ART-V and our method can generate sharp and temporally consistent videos while frames produced by TFGAN are blurry.
%     }
%     \label{fig:mug_txt_all}
% \end{subfigure}\hfill
% \begin{subfigure}[t] {1\linewidth}
%     \centering
%     \setlength{\tabcolsep}{0\linewidth}
%     \begin{tabular}{L{1\linewidth}}
%     \rowcolor{hlrowcolor}
%     \linespread{0.5}\noindent
%     \scriptsize	A female is wearing lipstick. This person has wavy hair and blond hair. She has high cheekbones, arched eyebrows and rosy cheeks. She has heavy makeup. She is young.
%     \end{tabular}
%     \includegraphics[width=1\linewidth]{cvpr2022/figure/vox_txt_all_5_color_new2.pdf}
%     \caption{Sample results on \textbf{Multimodal VoxCeleb}. Frame generated by ART-V at $t=1$ is sharp and clear, while  frames at later steps such as $t=5$ or $t=8$ are blurry.}
%     \label{fig:vox_txt_all}
% \end{subfigure}
% \caption{\textbf{Text-to-video} generation results for different methods on three datasets. Sample frames are shown at several time step ($t$). Conditioned text is provided at the top with light blue background.}
% \label{fig:text-to-video-all}
% \end{figure}
\begin{figure}[t]
\centering
\begin{subfigure}[t] {1\linewidth}
    \centering
    \setlength{\tabcolsep}{0\linewidth}
    \begin{tabular}{L{1\linewidth}}
    \rowcolor{hlrowcolor}
    \linespread{0.5}\noindent
    \small{\scriptsize A woman is making a surprise face.}
    \end{tabular}
    \includegraphics[width=\linewidth]{cvpr2022/figure/mug_txt_all_5_color_new2.pdf}
    \caption{Sample results on \textbf{MUG} dataset.
    ART-V and our method can generate sharp and temporally consistent videos while frames produced by TFGAN are blurry.
    }
    \label{fig:mug_txt_all}
\end{subfigure}\hfill
\begin{subfigure}[t] {1\linewidth}
    \centering
    \setlength{\tabcolsep}{0\linewidth}
    \begin{tabular}{L{1\linewidth}}
    \rowcolor{hlrowcolor}
    \linespread{0.5}\noindent
    \scriptsize	A female is wearing lipstick. This person has wavy hair and blond hair. She has high cheekbones, arched eyebrows and rosy cheeks. She has heavy makeup. She is young.
    \end{tabular}
    \includegraphics[width=1\linewidth]{cvpr2022/figure/vox_txt_all_5_color_new2.pdf}
    \caption{Sample results on \textbf{Multimodal VoxCeleb}. Frame generated by ART-V at $t=1$ is sharp and clear, while  frames at later steps such as $t=5$ or $t=8$ are blurry.}
    \label{fig:vox_txt_all}
\end{subfigure}
\caption{\textbf{Text-to-video} generation results for different methods. Sample frames are shown at several time steps ($t$). Conditioned text is provided at the top with light blue background.}
\label{fig:text-to-video-all}
\end{figure}
\begin{table}[h]
\caption{Classification accuracy (\%) on the Shapes dataset for video generation. Our method achieves the best performance.}
    \label{tab:shape_text}
    \centering
    % \scalebox{0.75}{
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{llcccccc}
    \toprule
    Condition & Methods & Shape & Color & Size & Motion & Dir & Avg \\
    \hline
    \multirow{3}{*}{Text Only} & TFGAN~\cite{tfgan} & 80.22 & \textbf{100.00} & 84.33 & \textbf{99.90} & \textbf{99.95} & 92.88 \\
    & ART-V & 95.07 & 98.68 & 97.71 & 92.72 & 96.04 & 96.04 \\ 
    &\cellcolor{hlrowcolor2}MMVID (Ours) &\cellcolor{hlrowcolor2}\textbf{95.56} &\cellcolor{hlrowcolor2}99.71 &\cellcolor{hlrowcolor2}\textbf{97.95} &\cellcolor{hlrowcolor2}97.80 &\cellcolor{hlrowcolor2}99.61 &\cellcolor{hlrowcolor2}\textbf{98.12} \\
    \hline\hline
    \multirow{2}{*}{Multimodal}
    & ART-V & 92.82 & 97.17 & 97.31 & 89.55 & 93.99 & 94.17 \\
    &\cellcolor{hlrowcolor2}MMVID (Ours) &\cellcolor{hlrowcolor2}\textbf{98.19} &\cellcolor{hlrowcolor2}\textbf{99.76} &\cellcolor{hlrowcolor2}\textbf{98.83} &\cellcolor{hlrowcolor2}\textbf{99.46} &\cellcolor{hlrowcolor2}\textbf{99.95} &\cellcolor{hlrowcolor2}\textbf{99.24} \\
    \bottomrule
    \end{tabular}}
    
\end{table}


% \begin{table}[h]
%     \centering
%     \scalebox{0.75}{
%     % \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lcccccc}
%     \toprule
%      & Shape & Color & Size & Motion & Direction & Average \\
%     \hline
%     ART-V & 92.82 & 97.17 & 97.31 & 89.55 & 93.99 & 94.17 \\
%     \todo{MMVID} (Ours)  & \textbf{98.19} & \textbf{99.76} & \textbf{98.83} & \textbf{99.46} & \textbf{99.95} & \textbf{99.24} \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Classification accuracies (\%) and FVD. ART-V and MMVID are both trained for 100k iterations.}
%     \label{tab:shape_text_vc}
% \end{table}

\subsection{Text-to-Video Generation}
% \noindent\textbf{Moving Shapes Dataset.} 
\noindent\textbf{Shapes}.
% Note that we train a classifier and retrain TFGAN model for the comparison as the original models are not released.
% Since we do not have the classifiers used in TFGAN, we retrain a TFGAN model for a fair comparison. We report the classification accuracies in Table~\ref{tab:shape_text}. 
We report the classification accuracy in Tab.~\ref{tab:shape_text} (top four rows) for the Shapes dataset. ART-V and MMVID are trained for $100$K iterations.
Compared with TFGAN~\cite{tfgan}, our model achieves significantly higher classification accuracy for Shape, Size, and Average (Avg) categories. Compared with ART-V, we perform better in all the categories.
% The low accuracy of Shape and Size for the generated samples from TFGAN can be verified in Fig.~\ref{fig:shape_txt_all}.
Note that our method has slightly lower accuracy on Color, Motion, and Direction (Dir) than TFGAN. The reason might be the VQGAN introduces errors in reconstruction, since the background is diverse and moving, and  it needs to encode these small translations by only $4\times4$ codes.
Note that to have a fair comparison, we do not apply text augmentation when performing comparison with other works.
% To have a fair comparison with other works, we do not apply text augmentation 
% Note that TFGAN has nearly perfect accuracies on color, motion, and direction. We think possible reason might be: (1) the pretrained classifier only has accuracies of \todo{xxx} on held-out test set, (2) the stage-I VQGAN model introduces errors in reconstruction, (given that the background is diverse and also moving, and the employed VQGAN model needs to encode these small translations by only $4 \times 4$ codes, this is reasonable). 
%  ART-V and MMVID are both trained for 100k iterations.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{cvpr2022/figure/shape_txt_all_color_new.pdf}
%     \setlength{\tabcolsep}{0\linewidth}
%     \hspace*{0.8em}\begin{tabular}
%         {C{0.12\linewidth}C{0.12\linewidth}C{0.12\linewidth}C{0.12\linewidth}C{0.12\linewidth}C{0.12\linewidth}C{0.12\linewidth}C{0.12\linewidth}}
%         \small$t=1$&\small$t=3$&\small$t=5$&\small$t=7$&\small$t=9$&\small\hspace{0.1cm}$t=11$&\small\hspace{0.1cm}$t=13$&\small\hspace{0.1cm}$t=15$
%     \end{tabular}
%     \caption{Text-to-video generation samples of TFGAN, ART-V, and our model at several time step ($t$). The conditioned text is provided at the top with light blue background. TFGAN cannot generate sequences with clear shape and complicated background.}
%     \label{fig:shape_txt_all}
% \end{figure}

\begin{table}[h]
\caption{Inception Score (IS) and classification accuracy (\%) on MUG for video generation. We mark `*' to IS values reported in TiVGAN. Our model achieves highest accuracy and IS.}
    \label{tab:mug_text}
    \centering
    \resizebox{1\linewidth}{!}{
    % \resizebox{1\linewidth}{!}{
    \begin{tabular}{llccc}
    \toprule
   Condition & Methods & Gender (\%) $\uparrow$ & Expression (\%) $\uparrow$ & IS $\uparrow$ \\
    \hline
    \multirow{7}{*}{Text Only}&TGAN~\cite{saito2017temporal}    & - & - & *4.63 \\
    &MoCoGAN~\cite{tulyakov2017mocogan} & - & - & *4.92 \\
     &TGANs-C~\cite{pan2017create} & - & - & *4.65 \\ 
     &TiVGAN~\cite{kim2020tivgan}  & - & - & *5.34 \\ 
     &TFGAN~\cite{tfgan} & 99.22 & \textbf{100.00} & 5.53 \\ 
   &ART-V & 93.46 & 99.12 & 5.72 \\ 
    &\cellcolor{hlrowcolor2}{MMVID} (Ours) &\cellcolor{hlrowcolor2}\textbf{99.90} &\cellcolor{hlrowcolor2}\textbf{100.00} &\cellcolor{hlrowcolor2}\textbf{5.94} \\ 
    \hline\hline
     \multirow{2}{*}{Multimodal} & ART-V & 89.16 & 98.54 & 5.59 \\
    &\cellcolor{hlrowcolor2}MMVID (Ours) &\cellcolor{hlrowcolor2}\textbf{98.14} &\cellcolor{hlrowcolor2}\textbf{100.00} &\cellcolor{hlrowcolor2}\textbf{5.85} \\ 
    \bottomrule
    \end{tabular}}
    
\end{table}
% \vspace{-0.1in}
\begin{table}[h]
\caption{Evaluation metrics for text-to-video generation on iPER and Multimodal VoxCeleb datasets.}
    \label{tab:vox_and_iper}
    \centering
    % \scalebox{0.9}{
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{llcccc}
    \toprule
    Dataset & Methods & CLIP $\uparrow$ & FVD $\downarrow$ & $F_8$ $\uparrow$ & $F_{1/8}$ $\uparrow$  \\
    \hline
    \multirow{2}{*}{iPER} & ART-V & - & 277.604 & 0.936 & 0.806  \\
    &\cellcolor{hlrowcolor2}MMVID (Ours) &\cellcolor{hlrowcolor2}- &\cellcolor{hlrowcolor2}\textbf{209.127} &\cellcolor{hlrowcolor2}\textbf{0.944} &\cellcolor{hlrowcolor2}\textbf{0.924}  \\ \hline\hline
    \multirow{1}{*}{Multimodal} & ART-V & 0.193 & 60.342 & 0.953 & 0.960  \\
    \multirow{1}{*}{VoxCeleb} &\cellcolor{hlrowcolor2}MMVID (Ours) &\cellcolor{hlrowcolor2}\textbf{0.197} &\cellcolor{hlrowcolor2}\textbf{46.763} &\cellcolor{hlrowcolor2}\textbf{0.972} &\cellcolor{hlrowcolor2}\textbf{0.971}  \\
    \bottomrule
    \end{tabular}}
    
\end{table}

\noindent\textbf{MUG}.
We follow the experimental setup in TiVGAN~\cite{kim2020tivgan} for experiments on the MUG expression dataset. 
We train models with a temporal step size of $8$ due to the memory limit of GPU. Note TiVGAN is trained with a step size of $4$ and generates $16$-frame videos, while our model generates $8$-frame videos in a single forward. We also train a 3D ConvNet as described in TiVGAN to evaluate the Inception Score and perform classification on Gender and Expression. Results are shown in Fig.~\ref{fig:mug_txt_all} and Tab.~\ref{tab:mug_text} (top 8 rows). Our model achieves the best performance.
% \begin{figure}[h]
%     \centering
%     % \includegraphics[width=\linewidth]{cvpr2022/figure/mug_txt_all_small.pdf}
%     \includegraphics[width=\linewidth]{cvpr2022/figure/mug_txt_all_5_color.pdf}
%     \setlength{\tabcolsep}{0\linewidth}
%     \hspace*{0.8em}\begin{tabular}{C{0.2\linewidth}C{0.2\linewidth}C{0.2\linewidth}C{0.2\linewidth}C{0.2\linewidth}}
%     % \small \hspace{1cm} $t=2$ &\small \hspace{0.6cm} $t=4$& \hspace{0.3cm} \small$t=6$&\small$t=8$
%     \small$t=1$ &\small\hspace{-0.1cm}$t=3$ &\small  \hspace{-0.2cm}$t=5$&\small\hspace{-0.3cm}$t=7$&\small\hspace{-0.5cm}$t=8$
%     \end{tabular}
%     \caption{Text-to-video generation samples on MUG at several time step ($t$). Conditioned text is given at the top.
%     ART-V and our method can generate sharp sharp and temporally consistent videos while frames produced by TFGAN are blurry.
%     }
%     \label{fig:mug_txt_all}
% \end{figure}

% \begin{table}[h]
%     \centering
%     % \scalebox{0.9}{
%     % \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lcccc}
%     \toprule
%      & CLIP $\uparrow$ & FVD $\downarrow$ & $F_8$ $\uparrow$ & $F_{1/8}$ $\uparrow$  \\
%     \hline
%                   ART-V & 0.193 & 60.342 & 0.953 & 0.960  \\
%     {MMVID} (Ours) & \textbf{0.197} & \textbf{46.763} & \textbf{0.972} & \textbf{0.971}  \\
%     \bottomrule
%     \end{tabular}%}
%     \caption{Evaluation metrics for text-to-video generation on Multimodal VoxCeleb dataset.}
%     \label{tab:vox_text}
% \end{table}
% \begin{table}[h]
%     \centering
%     % \scalebox{0.9}{
%     % \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lccc}
%     \toprule
%      & FVD $\downarrow$ & $F_8$ $\uparrow$ & $F_{1/8}$ $\uparrow$  \\
%     \hline
%              ART-V & 277.604 & 0.936 & 0.806  \\
%     {MMVID} (Ours) & \textbf{209.127} & \textbf{0.944} & \textbf{0.924}  \\
%     \bottomrule
%     \end{tabular}%}
%     \caption{Evaluation metrics for text-to-video generation on iPER dataset.}
%     \label{tab:iper_text}
% \end{table}

\noindent\textbf{iPER}. 
% To test the generalization capability of different models to unseen motions, we split a held-out set of $10$ videos ($186$ testing clips with each includes $100$ frames) which contains $10$ unique appearances performing A pose. 
We show the results of the dataset in Tab.~\ref{tab:vox_and_iper} (top 3 rows), demonstrating the advantages of our method. Long sequence generation results are shown in Fig.~\ref{fig:iper}.
% More visual samples are shown in Supplementary.

\noindent\textbf{Multimodal VoxCeleb}. We train ART-V and our model at a spatial resolution of $128\times128$ and a temporal step of $4$ to generate $8$ frames. Our method shows better results than ART-V on all the metrics, as shown in Tab.~\ref{tab:vox_and_iper} (bottom two rows). We notice ART-V can also generate video samples with good visual quality and are aligned well with the text descriptions. However, ART-V often produces samples that are not temporally consistent. For example, as shown in Fig.~\ref{fig:vox_txt_all}, the frame generated by ART-V at $t=1$ is sharp and clear, but frames at $t=5$ or $t=8$ are blurry. The reason might be the exposure bias in autoregressive models becomes more obvious as the sequence length is long, \emph{i.e.}, an $8$-frame video at resolution $128\times128$ has $512$ tokens. Thanks to bidirectional information during training and inference, our MMVID is able to produce temporally consistent videos. 
% We also train TFGAN at a spatial resolution of $64\times64$ and provide comparative results in Supplementary. %The samples are blurry and the results are given in  Supplementary  due to page limitations. 
% We also find simply drop out a few sentences from the text description can help the model to generate diverse samples.

% During training, we also find adding noise to textual information (text augmentation) by simply dropping out a few sentences from the text description helps the model to generate diverse samples.
% Quantitative metrics are given in Table~\ref{tab:vox_text}. 
%We evaluate the text-video relevance by CLIP score, which is computed as the cosine similarity of text embedding and image embedding of the first frame given by the pretrained CLIP model~\cite{radford2021learning}. We also compute the FVD score~\cite{unterthiner2018towards} from 2048 samples. Sample diversity is evaluated by the precision and recall distribution ($F_{8}$ and $F_{1/8}$)~\cite{precision_recall_distributions}. The  Human evaluation is the portion of AMTuker's preference given a pairwise comparison of samples.
% \begin{table}[h]
%     \centering
%     % \scalebox{0.9}{
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lccccc}
%     \toprule
%      & CLIP $\uparrow$ & FVD $\downarrow$ & $F_8$ $\uparrow$ & $F_{1/8}$ $\uparrow$ & Human \\
%     \hline
%     TFGAN & 413.301 & - & - & 0.363 & 0.279 \\
%     ART-V & - & - & - & - & - \\ \hline
%     \todo{MMVID} (Ours)  & - & - & - & - & - \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Evaluation metrics for text-to-video generation on VoxCeleb dataset.}
%     \label{tab:vox_text}
% \end{table}


% \begin{figure}[h]
%     \centering
%     % \includegraphics[width=1\linewidth]{cvpr2022/figure/vox_txt_all_new.pdf}
%     \includegraphics[width=1\linewidth]{cvpr2022/figure/vox_txt_all_5_color.pdf}
%     \setlength{\tabcolsep}{0\linewidth}
%     \hspace*{0.8em}\begin{tabular}{C{0.2\linewidth}C{0.2\linewidth}C{0.2\linewidth}C{0.2\linewidth}C{0.2\linewidth}}
    
%     % \small \hspace{1cm} $t=2$ &\small \hspace{0.6cm} $t=4$& \hspace{0.3cm} \small$t=6$&\small$t=8$
%     \small$t=1$ &\small\hspace{-0.1cm}$t=3$ &\small  \hspace{-0.3cm}$t=5$&\small\hspace{-0.3cm}$t=7$&\small\hspace{-0.5cm}$t=8$
%     \end{tabular}
%     \caption{Text-to-video generation samples on Multimodal VoxCeleb dataset. Frame generated by ART-V at $t=1$ is sharp and clear, while  frames at later steps such as $t=5$ or $t=8$ are blurry.}
%     \label{fig:vox_txt_all}
% \end{figure}

% \subsection{Application}
% We present various applications using our proposed framework. 
\begin{figure}[t]
\centering
\begin{subfigure}[t] {1\linewidth}
    \centering
    \setlength{\tabcolsep}{0\linewidth}
    \begin{tabular}{L{1\linewidth}}
    \rowcolor{hlrowcolor}\linespread{0.5}\noindent
    \small{\scriptsize	 A large green square is moving in a diagonal path in the northeast direction.} 
    \end{tabular}
    \includegraphics[width=1\linewidth]{cvpr2022/figure/shape_vc_color_new2.pdf}
    \caption{\textbf{Independent} multimodal control.
    The text description specifies the size, color, and shape of the object, and its motion. The visual control is a \emph{partially} observed image with its center masked out (shown as white), which provides control for the background. ART-V can generate correct object and motion, but suffers from incorporating consistent visual inputs such that the background is not temporal consistent. }
    \label{fig:shape_vc}
\end{subfigure}\hfill
\begin{subfigure}[t] {1\linewidth}
    \centering
    \setlength{\tabcolsep}{0\linewidth}
    \begin{tabular}{L{1\linewidth}}
    \rowcolor{hlrowcolor}
    \linespread{0.5}\noindent
    \small{\scriptsize	An object with color in image one, shape in image two, background in image three is moving in a diagonal path in the southwest direction.}
    \end{tabular}
    \includegraphics[width=1\linewidth]{cvpr2022/figure/shape_text_dep_4_color_new2.pdf}
    \caption{\textbf{Dependent} multimodal controls. The text description specifies from which image to extract color, shape, and background.}
    \label{fig:shape_text_dep}
\end{subfigure}
\caption{\textbf{Multimodal} generation results on Shapes with \emph{textual} (at top) and \emph{visual} ({first} column(s))  modalities. Sample frames are shown at several time step ($t$).}
\label{fig:multimodal-all}
\end{figure}
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.85\linewidth]{cvpr2022/figure/vox_vc_large_new2.pdf}
    \caption{\textbf{Independent and Dependent} multimodel video generation on Multimodal VoxCeleb with textual control (TC), image control (IC), and video control (VC). \emph{Row (a) - (b)}: TC + IC (segmentation mask); \emph{Row (c)}: TC (null) + IC (drawing); \emph{Row (d) - (e)}: dependent TC + IC; \emph{Row (f) - (h)}: TC + IC (partial image) and the TC of (g) is obtained from the TC of (f) by replacing ``blond'' with ``black''; \emph{Row (i)}: dependent TC + VC and the VC includes content and motion information. }
    \label{fig:vox_vc}
\end{figure*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{cvpr2022/figure/iper_app2.pdf}
    \caption{\textbf{Extrapolation and Interpolation}. \emph{Row (a) - (b)}: long sequence generation via extrapolation. 
    % The real sequences of (a) and (b) are held out from the training set so that there is no training data with the appearance in (a) and (b) performing the same motion.
    \emph{Row (c)}: interpolating a real sequence. Frames in dotted red boxes are fixed as preservation control. Textual controls for each row are: (a) ``Person 024 dressed in 2 is performing random pose, normal speed.''; (b) ``Person 024 dressed in 1 is performing A-pose, normal speed.''; and (c) ``Person 028 dressed in 2 is performing A-pose, normal speed.''}
    \label{fig:iper}
\end{figure*}


\subsection{Multimodal Video Generation}
\noindent Multimodal conditions can evolved in two cases: independent and dependent, and we show experiments on both.

\noindent\textbf{Independent Multimodal  Controls}. This setting is similar to conventional conditional video generation, except the condition is changed to multimodal controls.
We conduct experiments on Shapes and MUG datasets with the input condition as the combination of text and image. The bottom two rows in Tab.~\ref{tab:shape_text} and Tab.~\ref{tab:mug_text} demonstrate the advantages of our method over ART-V on all metrics. Additionally, we provide generated samples in Fig.~\ref{fig:shape_vc}, where only a \emph{partial} image is given as the visual condition. As can be seen, ART-V cannot satisfy the visual constraint well and the generated video is not consistent. 
% than the one without image control (Fig.~\ref{fig:shape_txt_all}). 
The quality degradation for multimodal video synthesis of ART-V can also be verified in Tab.~\ref{tab:shape_text} as it shows lower classification accuracy than text-only generation, while our method is able to generate high quality videos for different condition signals.
% , including text only, multimodal, and partial visual and textual condition.

We also conduct extensive experiments of video generation under various combinations of textual and image controls on Multimodal VoxCeleb, as shown in Fig.~\ref{fig:vox_vc}. We apply three different image controls, including segmentation mask (Fig.~\ref{fig:vox_vc} row (a) - (b)), drawing (Fig.~\ref{fig:vox_vc} row (c) - (d)), and partial image (Fig.~\ref{fig:vox_vc} row (d) - (f)).  In Fig.~\ref{fig:vox_vc} row (b), our method can synthesize frames with eyeglasses even though eyeglasses are not shown in segmentation mask. In  Fig.~\ref{fig:vox_vc} row (f) - (g), we show that using the same image control while  replacing the ``blond'' with ``black'' in the text description, we can generate frames with similar content except the hair color is changed. Such examples demonstrate that our method has a good understanding of multimodal controls.

% Three settings are considered: (1) text and segmentation mask, (2) text and drawing, (3) text and partial image. Samples are shown in Fig.~\ref{fig:vox_vc}, in row (b), our model generates frames with eyeglasses even though `eyeglasses' is not shown in the segmentation mask.
% condition on image controls and achieves higher accuracy.
% where the conditional information can be multi-modal. For Shapes dataset, we evaluate and report classification accuracies in bottom two rows Tab.~\ref{tab:shape_text}. For MUG dataset, we report gender and expression classification accuracies and IS in bottom two rows of Tab.~\ref{tab:mug_text}. Our proposed MMVID performs better than ART-V in all metrics and datasets. Fig.~\ref{fig:shape_vc} shows samples of ART-V and MMVID where partially observed images are given as visual control. As shown, ART-V cannot satisfy the visual constraint well and the generated video becomes less consistent than without image control (Fig.~\ref{fig:shape_txt_all}. This can be verified by the lower accuracies. On the contrary, MMVID is able to condition on image controls and achieves higher accuracy.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{cvpr2022/figure/shape_vc_color.pdf}
%     \setlength{\tabcolsep}{0\linewidth}
%     \vspace{-0.7em}
%     \hspace*{3.8em}\begin{tabular}
%         {C{0.1\linewidth}C{0.1\linewidth}C{0.1\linewidth}C{0.1\linewidth}R{0.1\linewidth}R{0.12\linewidth}C{0.12\linewidth}C{0.12\linewidth}}
%         \tiny$t=1$&\tiny$t=3$&\hspace{0.5em}\tiny$t=5$&\hspace{0.5em}\tiny$t=7$&\tiny$t=9$&\tiny$t=11$&\hspace{0.2em}\tiny$t=13$&\hspace{-0.3em}\tiny$t=15$
%     \end{tabular}
%     \caption{Multimodal video generation on Shapes dataset with visual (\emph{first} column) and textual (at top) modalities.
%     The text description specifies the size, color, and shape of the object, as well as its motion. The visual control is a \emph{partially} observed image with its center masked out (shown as white), which provides control for the background. ART-V can generate correct object and motion, but suffers from incorporating consistent visual control.}
%     \label{fig:shape_vc}
% \end{figure}
% \begin{table}[h]
%     \centering
%     \scalebox{0.75}{
%     % \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lcccccc}
%     \toprule
%      & Shape & Color & Size & Motion & Direction & Average \\
%     \hline
%     ART-V & 92.82 & 97.17 & 97.31 & 89.55 & 93.99 & 94.17 \\
%     \todo{MMVID} (Ours)  & \textbf{98.19} & \textbf{99.76} & \textbf{98.83} & \textbf{99.46} & \textbf{99.95} & \textbf{99.24} \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Classification accuracies (\%) and FVD. ART-V and MMVID are both trained for 100k iterations.}
%     \label{tab:shape_text_vc}
% \end{table}
% \begin{table}[h]
%     \centering
%     % \scalebox{1}{
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lccc}
%     \toprule
%     % \multicolumn{1}{l}{} & \multicolumn{2}{c}{Accuracy (\%) $\uparrow$} & \multicolumn{1}{c}{IS $\uparrow$} \\
%     % \cmidrule(lr){2-3}
%     %  & Gender & Expression &  \\
%     & Gender (\%) $\uparrow$ & Expression (\%) $\uparrow$ & IS $\uparrow$ \\
%     \hline
%     ART-V & 89.16 & 98.54 & 5.59 \\
%     \todo{MMVID} (Ours) & \textbf{98.14} & \textbf{100.00} & \textbf{5.85} \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{Inception Score and classification accuracies on MUG dataset.}
%     \label{tab:mug_text_vc}
% \end{table}

\noindent\textbf{Dependent Multimodal Controls}. Furthermore, we introduce a novel task for multimodal video generation where textual and visual controls are dependent, such that the actual control signals are guided by the textual description. For example, Fig.~\ref{fig:shape_text_dep} illustrates how the text informs from which image  the model should query color, shape, and background information. More synthesized examples on Multimodal VoxCeleb are given in Fig.~\ref{fig:vox_vc}. For Fig.~\ref{fig:vox_vc} row (d) - (e), 
% our method can synthesize high fidelity videos even with partially observed visual controls.   
our model learns to combine detailed facial features from drawing or image and coarse features (\emph{i.e.}, pose) from mask.
For Fig.~\ref{fig:vox_vc} row (i), our method successfully retargets the subject with an appearance from the given image control (IC1) and generates frames with the motion specified by consecutive images that provide motion control (VC1).



\begin{table}[h]
    \caption{Analysis on Shapes for video augmentation strategies.
    % The strategies are uniformly chosen when more than one is used. All models are trained with $\lambda_\text{MSM}=4$ for $90$K iterations.
    }
    \label{tab:ablation_vid}
    \centering
    % \scalebox{0.75}{
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{cccccccccc}
    \toprule
    \multicolumn{4}{c}{Video Augmentation} & \multicolumn{6}{c}{Accuracy (\%)}\\
    \cmidrule(lr){1-4} \cmidrule(lr){5-10}
    Swap & Shuffle & Color & Affine & Shape & Color & Size & Motion & Dir & Avg \\
    \hline
    \redxmark & \redxmark & \redxmark & \redxmark & 90.43 & 89.07 & 95.61 & 92.48 & 99.13 & 93.34 \\
    \greencmark & \redxmark & \redxmark & \redxmark & 91.02 & 89.84 & 93.75 & 91.02 & 98.05 & 92.73 \\
    \redxmark & \greencmark & \redxmark & \redxmark & 88.28 & 89.45 & 94.53 & 88.28 & 98.44 & 91.80 \\
    \redxmark & \redxmark & \greencmark & \redxmark & 91.80 & {\bf 91.02} & 94.53 & 93.36 & 98.83 & 93.91 \\
    \redxmark & \redxmark & \redxmark & \greencmark & 90.62 & 90.62 & 95.31 & 89.84 & 98.83 & 93.05 \\
    \rowcolor{hlrowcolor2}
    \greencmark & \greencmark & \greencmark & \greencmark & {\bf 93.36} & 88.28 & {\bf 95.70} & {\bf 93.75} & {\bf 99.61} & {\bf 94.14} \\
    \bottomrule
    \end{tabular}}

\end{table}
\subsection{Long Sequence Generation and Ablation}
\noindent\textbf{Long Sequence Generation}.
Our approach enables temporal extrapolation of videos. We show samples of video extrapolation and interpolation in Fig.~\ref{fig:iper}. Samples from Fig.~\ref{fig:iper} row (a) - (b) are generated by being iteratively conditioned on previous $6$ frames to generate the following $2$ frames. Fig.~\ref{fig:iper} row (c) shows an example of synthesizing one frame by interpolating two consecutive real frames.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{cvpr2022/figure/vox_lang_new.pdf}
    \caption{\textbf{Analysis on language embedding}. Samples are generated with out-of-distribution textual inputs.
    We reword the original text (strikethrough) with equivalent descriptions (italic) that do not exist in the training.
    We show the first frames from the generated sequences for each method. Frames generated using the pretrained language model (\emph{w/} RoBERTa) is more correlated with text inputs.}
    \label{fig:vox_lang}
\end{figure}
% \subsection{Ablation Study}
\noindent\textbf{Analysis on VID Task}. We perform analysis for different \texttt{VID} strategies on the Shapes dataset. Tab.~\ref{tab:ablation_vid} shows that the highest average accuracy is achieved when all augmentation is used (sampled uniformly).
% , thus we fix this as a hyperparameter in later experiments. 
% We ablate the use of different \texttt{VID} strategies on Shapes dataset in our early experiments. As shown in Tab.~\ref{tab:ablation_vid}, the highest average accuracy is achieved when all video augmentation is used (sampled uniformly), thus we fix this as a hyperparameter in later experiments. 
Also note that accuracy for color is the highest when we only apply color augmentation. 
% User study of comparisons among ART-V, MMVID and MMVID with text augmentation (MMVID-TA), and ablation of constructing negative \texttt{REL} sequence are given in Supplementary. 

\noindent\textbf{Analysis on Language Embedding}.  Analysis of using a pretrained language model is shown in Fig.~\ref{fig:vox_lang}. The method with a language model (\emph{w/} RoBERTa) is more robust to various text inputs than the one without it (\emph{w/o} RoBERTa).
% ablation: real lauguage vs categorization (clip and human) MMVID-TA is MMVID with text augmentation. Tab.~\ref{tab:vox_amt} and Fig.~\ref{fig:vox_lang}

% \begin{table}[h]
%     \centering
%     % \scalebox{0.75}{
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{cccccccccc}
%     \toprule
%     \multicolumn{4}{c}{Video Augmentation} & \multicolumn{6}{c}{Accuracy (\%)}\\
%     \cmidrule(lr){1-4} \cmidrule(lr){5-10}
%     Swap & Shuffle & Color & Affine & Shape & Color & Size & Motion & Dir & Avg \\
%     \hline
%     %\redxmark & \redxmark & \redxmark & \redxmark & 90.23 & 90.23 & 96.78 & 92.77 & 99.02 & 93.81 \\
%     \greencmark & \redxmark & \redxmark & \redxmark & 91.02 & 89.84 & 93.75 & 91.02 & 98.05 & 92.73 \\
%     \redxmark & \greencmark & \redxmark & \redxmark & 88.28 & 89.45 & 94.53 & 88.28 & 98.44 & 91.80 \\
%     \redxmark & \redxmark & \greencmark & \redxmark & 91.80 & {\bf 91.02} & 94.53 & 93.36 & 98.83 & 93.91 \\
%     \redxmark & \redxmark & \redxmark & \greencmark & 90.62 & 90.62 & 95.31 & 89.84 & 98.83 & 93.05 \\
%     \rowcolor{hlrowcolor2}
%     \greencmark & \greencmark & \greencmark & \greencmark & {\bf 93.36} & 88.28 & {\bf 95.70} & {\bf 93.75} & {\bf 99.61} & {\bf 94.14} \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ablation analysis on the Shapes dataset for different video augmentation strategies. The strategies are uniformly chosen when more than one is used. All models are trained with $\lambda_\text{MSM}=4$ for $90$K iterations.
%     % Classification accuracy (\%) on the Shapes dataset for video generation. We ablate different video augmentation strategies. When all augmentations are used, they are chosen uniformly for each sample. Models are trained with $\lambda_\text{MSM}=4$ for 90K iterations.
%     }
%     \label{tab:ablation_vid}
% \end{table}
% \begin{table}[h]
%     \centering
%     % \scalebox{0.9}{
%     % \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lccccc}
%     \toprule
%      & FVD $\downarrow$ & $F_8$ $\uparrow$ & $F_{1/8}$ $\uparrow$  \\
%     \hline
%              ART-V &  & 60.342 & 0.953 & 0.960  \\
%     {MMVID} (Ours) & \textbf{0.197} & \textbf{46.763} & \textbf{0.972} & \textbf{0.971}  \\
%     \bottomrule
%     \end{tabular}%}
%     \caption{Evaluation metrics for text-to-video generation on Multimodal VoxCeleb dataset.}
%     \label{tab:ablation_rel}
% \end{table}


==> cvpr2022/6_conclusion.tex <==
% \section{Limitation}
% % \textbf{Limitation.} 
% Here we briefly summarize three limitation of our method. More details can be found in the Appendix.
% \emph{Higher Resolution Generation}. 
% We perform experiments for generating higher resolution videos. However, we notice worse temporal consistency than videos generated at lower resolution. Applying an image-level consistent regularization constraint might be helpful to better temporal consistency. \emph{Longer Sequence Generation}. We notice the extrapolation in longer sequence generation might not always give reasonable motion patterns. To alleviate this, it might be helpful to balance training set with diverse motion patterns. \emph{Diversity of Non-Autoregressive Transformer}. We notice the autogressive transformer might generate more diverse videos, compared with the non-autoregressive transformer, though the quality is worse. An interesting direction is to study how to futher improve the diversity of non-autoregressive transformer.


\section{Limitation and Conclusion}
% This paper targets a new problem, which is video generation using multimodal inputs. To tackle the problem, we utilize a two-stage video generation framework that includes an autoencoder for quantized representation of images and videos and a non-autoregressive transformer for predicting video tokens from multimodal input signals. Several techniques are proposed, including the special \texttt{VID} token, textual embedding, and improved mask prediction, to help generate temporally consistent videos. 
% % With our approach, various applications can be built, such as video interpolation and extrapolation for long sequence generation, and dependent multimodal generation with various visual controls. 
% On the other hand, the proposed method also contains some limitation, including temporal consistency issues for high resolution videos, how to generate diverse motion patterns for longer sequences, and how to further improve the diversity of non-autoregressive transformer. More details can be found in the Appendix. Besides improving the limitation, a future direction might be how to leverage more control modalities, such as audio, to generate videos with a much higher resolution. 
This paper targets a new problem, which is video generation using multimodal inputs. To tackle the problem, we utilize a two-stage video generation framework that includes an autoencoder for quantized representation of images and videos and a non-autoregressive transformer for predicting video tokens from multimodal input signals. Several techniques are proposed, including the special \texttt{VID} token, textual embedding, and improved mask prediction, to help generate temporally consistent videos. 
On the other hand, the proposed method also contains some limitations, including temporal consistency issues for high-resolution videos, generating diverse motion patterns for longer sequences, and further improving the diversity of non-autoregressive transformers. More details can be found in the Appendix. Besides improving the limitation, a future direction might be to leverage more control modalities, such as audio, to generate videos with a much higher resolution. 

==> cvpr2022/authors.tex <==
\author{Ligong Han\affmark[1]\affmark[2]\thanks{Work done during an internship at Snap Inc. }\quad\quad
\quad Jian Ren\affmark[1]\quad\quad Hsin-Ying Lee\affmark[1] \quad\quad
Francesco Barbieri\affmark[1]\quad\quad \\ Kyle Olszewski\affmark[1]\quad\quad Shervin Minaee\affmark[1] \quad\quad Dimitris Metaxas\affmark[2] \quad\quad Sergey Tulyakov\affmark[1]\\
{\affmark[1]Snap Inc.\quad\quad\quad\affmark[2]Rutgers University }
}


==> cvpr2022/limitation_section.tex <==
\section{Limitation and Future Work}
\noindent\textbf{Higher Resolution Generation}.
We conduct experiments to generate higher resolution videos.

by performing experiments on the Multimodal VoxCeleb dataset to synthesize video with the resolution of $256\times256$. Synthesized videos for the task of text-to-video generation are shown in Fig.~\ref{fig:more_vox_our_256}. We notice that artifacts can be found from some videos: \eg we find synthesized samples are more likely to show weird colors (Fig.~\ref{fig:more_vox_our_256}, the third row and the second sample) or appear to be blurry (Fig.~\ref{fig:more_vox_our_256} the last row and the second and the fourth sample). We also find that the temporal consistency is worse than videos generated at the resolution of $128\times128$. One possible reason might be that each frame at a higher resolution requires a longer token sequence. Therefore, an image-level temporal regularization constraint might be necessary to improve the video consistency, which we leave for future work.

\noindent\textbf{Longer Sequence Generation}. For the task of long sequence generation, we notice that extrapolation might not always give reasonable motion patterns. For example, as shown in Fig.~\ref{fig:more_iper_our_long}, the textual inputs from the first row struggle to generate diverse motions when the speed is given as ``slow''. This might be due to the temporal step size used to sample frames during training being short when the speed is ``slow'' and the frames cannot always cover diverse motion patterns.  A future direction could be balancing the training set to cover enough motion patterns for the sampled frames. 

\noindent\textbf{Diversity of Non-Autoregressive Transformer}. Compared with the autoregressive transformer, the non-autoregressive transformer can generate videos with better temporal consistency. However, we notice that the autoregressive transformer might generate more diverse videos, though many have low video quality. We apply text augmentation and improved mask-predict to improve the diversity of the non-autoregressive transformer. An interesting research direction is how to unify the training methods from the autoregressive and non-autoregressive transformer to enhance the non-autoregressive transformer itself for generating more diverse videos. We leave the direction as to future work.
